Evalet: Evaluating Large Language Models through Functional Fragmentation

Practitioners increasingly rely on Large Language Models (LLMs) to evaluate generative AI outputs through "LLM-as-a-Judge" approaches. However, these methods produce holistic scores that obscure which specific elements influenced the assessments. We propose functional fragmentation, a method that dissects each output into key fragments and interprets the rhetoric functions that each fragment serves relative to evaluation criteria -- surfacing the elements of interest and revealing how they fulfill or hinder user goals. We instantiate this approach in Evalet, an interactive system that visualizes fragment-level functions across many outputs to support inspection, rating, and comparison of evaluations. A user study (N=10) found that, while practitioners struggled to validate holistic scores, our approach helped them identify 48% more evaluation misalignments. This helped them calibrate trust in LLM evaluations and rely on them to find more actionable issues in model outputs. Our work shifts LLM evaluation from quantitative scores toward qualitative, fine-grained analysis of model behavior.

==> tables/tech_fragment.tex <==
\begin{table}[t!]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Method}       & \textbf{IoU}   & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    \\ \midrule
\textbf{\texttt{Ours}}  & \textbf{0.543} & 0.607     & \textbf{0.902}  & \textbf{0.726} \\
\textbf{\texttt{Rating}} & 0.414          & \textbf{0.615}              & 0.843           & 0.711          \\ \bottomrule
\end{tabular}%
\caption{Performance of the tested methods in fragment extraction as measured by the Intersection-over-Union (IoU) of predicted and ground-truth fragments, and precision, recall, and F1-score of the predicted fragments.}
\Description{This table compares the performance of two methods, Ours and Rating, in fragment extraction. It reports four metrics: Intersection-over-Union (IoU), Precision, Recall, and F1-score.
Our method achieves higher IoU (0.543 vs. 0.414) and Recall (0.902 vs. 0.843), while Rating method shows slightly higher Precision (0.615 vs. 0.607). Overall, our approach obtains the best F1-score of 0.726 compared to 0.711 for the baseline.}
\label{tab:tech_fragment}
\end{table}

==> tables/tech_overall.tex <==
\begin{table}[t]
\centering
\begin{tabular}{@{}lcccc@{}}
\toprule
\textbf{Method}       & \textbf{Overall} & \textbf{Chat}  & \textbf{Chat-Hard} & \textbf{Safety} \\ \midrule
\textbf{\texttt{Ours}}  & \textbf{0.801}            & \textbf{0.842} & \textbf{0.559}              & \textbf{0.849}           \\
\textbf{\texttt{Rating}} & 0.755   & 0.741          & 0.529     & 0.831  \\ \bottomrule
\end{tabular}%
\caption{Performance of the tested methods in terms of their accuracy at identifying the higher quality outputs from a pair of LLM-generated outputs. The table shows the accuracy for the whole dataset and for each subset.}
\Description{This table evaluates the accuracy of two methods, Ours and Rating, at selecting higher-quality outputs from LLM-generated pairs. The evaluation is reported across four settings: Overall, Chat, Chat-Hard, and Safety. Our method outperforms the baseline in all categories, achieving the highest accuracy overall (0.801 vs. 0.755), as well as in Chat (0.842 vs. 0.741), Chat-Hard (0.559 vs. 0.529), and Safety (0.849 vs. 0.831).}
\label{tab:tech_overall}
\end{table}
